Novelty-based Generalization Evaluation for Traffic Light Detection

The advent of Convolutional Neural Networks (CNNs) has led to their application in several domains. One noteworthy application is the perception system for autonomous driving that relies on the predictions from CNNs. Practitioners evaluate the generalization ability of such CNNs by calculating various metrics on an independent test dataset. A test dataset is often chosen based on only one precondition, i.e., its elements are not a part of the training data. Such a dataset may contain objects that are both similar and novel w.r.t. the training dataset. Nevertheless, existing works do not reckon the novelty of the test samples and treat them all equally for evaluating generalization. Such novelty-based evaluations are of significance to validate the fitness of a CNN in autonomous driving applications. Hence, we propose a CNN generalization scoring framework that considers novelty of objects in the test dataset. We begin with the representation learning technique to reduce the image data into a low-dimensional space. It is on this space we estimate the novelty of the test samples. Finally, we calculate the generalization score as a combination of the test data prediction performance and novelty. We perform an experimental study of the same for our traffic light detection application. In addition, we systematically visualize the results for an interpretable notion of novelty.

==> deprecated.tex <==
\section{Experimental evaluations}\label{sec:experimental_eval} 

\begin{table}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
      & \multicolumn{2}{c}{Red} & \multicolumn{2}{c}{Yellow} & \multicolumn{2}{c}{Green} \\ \midrule
      & Train      & Test       & Train        & Test        & Train       & Test        \\
BSTLD & 3977       & 5252       & 419          & 154         & 5225        & 7454        \\
DTLD  & 19776      & 15765      & 1444         & 2946        & 25006       & 29874       \\ \bottomrule
\end{tabular}
}
\end{table}
\subsection{Generalization comparison for TL detector}

\subsection{Contamination of data labels}
\begin{table*}
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{cccccccc@{}}
\toprule
True class & Contamination class & Algorithm & \multicolumn{5}{c}{\begin{tabular}[c]{@{}c@{}}Contamination \%\end{tabular}} \\ \midrule
           &     &  & 2 & 4 & 6 & 8 & 10 \\ \cmidrule{4-8}
     Green &                Red &             LOF &       0.98±0.01 &    \textbf{1}±0.0 &   0.99±0.0 &   0.99±0.0 &   0.99±0.0 \\
           &                  &             ISO &       0.68±0.03 &  0.68±0.01 &   0.7±0.01 &  0.69±0.01 &  0.68±0.01 \\
           &                  &           OCSVM &       0.93±0.01 &   0.94±0.0 &   0.93±0.0 &  0.93±0.01 &   0.94±0.0 \\
           &                  &            ABOD &       0.94±0.02 &   0.97±0.0 &   0.96±0.0 &  0.96±0.01 &   0.96±0.0 \\
           &                  &             SOD &       0.69±0.01 &  0.61±0.01 &  0.57±0.02 &  0.54±0.01 &   0.54±0.0 \\
           &                  &            LODA &       0.79±0.03 &   0.83±0.0 &  0.86±0.01 &  0.84±0.01 &   0.76±0.0 \\
           &                  &             COF &       0.56±0.04 &  0.48±0.01 &  0.47±0.02 &  0.47±0.01 &  0.46±0.01 \\
           &                  &  Feature-bagging &         \textbf{1}±0.0 &    \textbf{1}±0.0 &    \textbf{1}±0.0 &    \textbf{1}±0.0 &    \textbf{1}±0.0 \\
           &                  &             MCD &        0.8±0.03 &   0.82±0.0 &  0.82±0.01 &  0.81±0.01 &   0.82±0.0 \\
           &                  &            LSCP &       0.99±0.01 &    \textbf{1}±0.0 &   0.99±0.0 &   0.99±0.0 &   0.99±0.0 \\  \cmidrule{2-8}
           &             Yellow &             LOF &         \textbf{1}±0.0 &          X &          X &          X &          X \\
           &               &             ISO &        0.73±0.0 &          X &          X &          X &          X \\
           &               &           OCSVM &        0.94±0.0 &          X &          X &          X &          X \\
           &               &            ABOD &        0.98±0.0 &          X &          X &          X &          X \\
           &               &             SOD &       0.58±0.01 &          X &          X &          X &          X \\
           &               &            LODA &        0.82±0.0 &          X &          X &          X &          X \\
           &               &             COF &       0.41±0.01 &          X &          X &          X &          X \\
           &               &  Feature-bagging &        0.99±0.0 &          X &          X &          X &          X \\
           &               &             MCD &        0.84±0.0 &          X &          X &          X &          X \\
           &               &            LSCP &        0.97±0.0 &          X &          X &          X &          X \\  \cmidrule{2-8}
       Red &              Green &             LOF &        0.99±0.0 &   0.99±0.0 &   0.99±0.0 &   0.99±0.0 &   0.99±0.0 \\
           &                &             ISO &       0.66±0.03 &  0.65±0.01 &  0.66±0.01 &  0.65±0.01 &  0.66±0.01 \\
           &                &           OCSVM &       0.75±0.01 &  0.73±0.01 &  0.73±0.02 &  0.73±0.01 &  0.74±0.01 \\
           &                &            ABOD &       0.93±0.01 &   0.92±0.0 &  0.92±0.01 &  0.92±0.01 &  0.92±0.01 \\
           &                &             SOD &        0.9±0.01 &   0.84±0.0 &  0.82±0.01 &  0.81±0.01 &  0.78±0.01 \\
           &                &            LODA &       0.72±0.03 &  0.71±0.02 &  0.72±0.02 &   0.7±0.01 &  0.74±0.01 \\
           &                &             COF &       0.67±0.04 &  0.57±0.02 &   0.5±0.01 &    0.5±0.0 &  0.49±0.01 \\
           &                &  Feature-bagging &         \textbf{1}±0.0 &   0.99±0.0 &   0.99±0.0 &   0.99±0.0 &   0.99±0.0 \\
           &                &             MCD &       0.88±0.02 &  0.87±0.01 &  0.86±0.01 &  0.86±0.01 &  0.87±0.01 \\
           &                &            LSCP &       0.97±0.01 &   0.97±0.0 &  0.96±0.01 &  0.97±0.01 &   0.96±0.0 \\  \cmidrule{2-8}
           &             Yellow &             LOF &         \textbf{0.9}±0.0 &          X &          X &          X &          X \\
           &               &             ISO &        0.62±0.0 &          X &          X &          X &          X \\
           &               &           OCSVM &       0.74±0.01 &          X &          X &          X &          X \\
           &               &            ABOD &        0.76±0.0 &          X &          X &          X &          X \\
           &               &             SOD &        0.72±0.0 &          X &          X &          X &          X \\
           &               &            LODA &       0.63±0.01 &          X &          X &          X &          X \\
           &               &             COF &       0.45±0.03 &          X &          X &          X &          X \\
           &               &  Feature-bagging &       0.87±0.01 &          X &          X &          X &          X \\
           &               &             MCD &         0.8±0.0 &          X &          X &          X &          X \\
           &               &            LSCP &        0.78±0.0 &          X &          X &          X &          X \\  \cmidrule{2-8}
    Yellow &              Green &             LOF &       0.93±0.09 &  0.99±0.01 &  0.96±0.05 &  0.98±0.02 &  0.99±0.01 \\
           &                &             ISO &        0.84±0.1 &  0.79±0.08 &  0.74±0.09 &  0.71±0.07 &  0.79±0.04 \\
           &                &           OCSVM &       0.95±0.05 &  0.99±0.01 &  0.99±0.01 &  0.96±0.04 &  0.97±0.01 \\
           &                &            ABOD &       0.95±0.06 &  0.89±0.08 &  0.93±0.05 &  0.98±0.02 &  0.92±0.07 \\
           &                &             SOD &       0.99±0.01 &  0.97±0.01 &  0.89±0.01 &  0.84±0.06 &   0.9±0.01 \\
           &                &            LODA &        0.72±0.1 &  0.87±0.04 &  0.86±0.02 &  0.81±0.05 &  0.87±0.04 \\
           &                &             COF &         \textbf{1}±0.0 &    1.0±0.0 &    1.0±0.0 &    1.0±0.0 &    1.0±0.0 \\
           &                &  Feature-bagging &         \textbf{1}±0.0 &  0.99±0.01 &  0.99±0.01 &  0.99±0.01 &  0.99±0.01 \\
           &                &             MCD &       0.86±0.09 &   0.81±0.1 &  0.78±0.12 &  0.83±0.04 &  0.81±0.08 \\
           &                &            LSCP &        0.9±0.15 &  0.98±0.01 &  0.93±0.05 &   0.91±0.1 &  0.93±0.01 \\  \cmidrule{2-8}
           &                Red &             LOF &       0.89±0.08 &  0.94±0.07 &  0.98±0.01 &  0.97±0.03 &  0.96±0.02 \\
           &                  &             ISO &       0.55±0.07 &  0.53±0.09 &  0.78±0.03 &  0.72±0.02 &   0.71±0.1 \\
           &                  &           OCSVM &       0.92±0.08 &  0.95±0.01 &  0.97±0.02 &  0.95±0.02 &  0.97±0.03 \\
           &                  &            ABOD &       0.74±0.19 &  0.88±0.09 &  0.94±0.04 &  0.94±0.04 &  0.89±0.05 \\
           &                  &             SOD &       0.98±0.02 &  0.96±0.01 &   0.9±0.02 &  0.91±0.03 &  0.81±0.06 \\
           &                  &            LODA &       0.74±0.04 &  0.77±0.02 &   0.78±0.0 &  0.74±0.03 &  0.79±0.08 \\
           &                  &             COF &         \textbf{1}±0.0 &    1.0±0.0 &    1.0±0.0 &    1.0±0.0 &    1.0±0.0 \\
           &                  &  Feature-bagging &       0.91±0.07 &  0.96±0.06 &  0.99±0.01 &  0.99±0.02 &  0.98±0.01 \\
           &                  &             MCD &       0.55±0.14 &  0.51±0.05 &  0.77±0.05 &  0.74±0.04 &   0.74±0.1 \\
           &                  &            LSCP &       0.78±0.15 &  0.86±0.04 &  0.91±0.03 &  0.95±0.03 &  0.93±0.04 \\
      \bottomrule
\end{tabular}
}
\caption{BSTLD outlier detection algorithms benchmark}
\end{table*}

\begin{table*}
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{cccccccc@{}}
\toprule
True class & Contamination class & Algorithm & \multicolumn{5}{c}{\begin{tabular}[c]{@{}c@{}}Contamination \%\end{tabular}} \\ \midrule
           &     &  & 2 & 4 & 6 & 8 & 10 \\ \cmidrule{4-8}
Green &                Red &             LOF &       0.94±0.01 &   0.95±0.0 &   0.95±0.0 &   0.94±0.0 &   0.95±0.0 \\
           &                  &             ISO &       0.82±0.01 &   0.82±0.0 &   0.83±0.0 &  0.82±0.01 &   0.81±0.0 \\
           &                  &           OCSVM &        0.86±0.0 &   0.86±0.0 &   0.87±0.0 &   0.86±0.0 &   0.86±0.0 \\
           &                  &            ABOD &       0.82±0.01 &   0.83±0.0 &   0.83±0.0 &  0.83±0.01 &   0.83±0.0 \\
           &                  &             SOD &       0.74±0.01 &   0.72±0.0 &   0.7±0.01 &   0.68±0.0 &  0.68±0.01 \\
           &                  &            LODA &       0.84±0.01 &   0.85±0.0 &   0.84±0.0 &   0.85±0.0 &   0.86±0.0 \\
           &                  &             COF &       0.78±0.01 &  0.73±0.01 &   0.69±0.0 &   0.66±0.0 &   0.64±0.0 \\
           &                  &  Feature-bagging &        0.93±0.0 &   0.93±0.0 &   0.93±0.0 &   0.93±0.0 &   0.93±0.0 \\
           &                  &             MCD &       0.83±0.01 &   0.83±0.0 &   0.83±0.0 &   0.83±0.0 &   0.84±0.0 \\
           &                  &            LSCP &       0.95±0.01 &   0.95±0.0 &   0.95±0.0 &   0.95±0.0 &   0.95±0.0 \\ \cmidrule{2-8}
           &             Yellow &             LOF &        0.93±0.0 &   0.93±0.0 &   0.93±0.0 &   0.92±0.0 &          X \\
           &               &             ISO &        0.8±0.01 &   0.81±0.0 &   0.81±0.0 &   0.81±0.0 &          X \\
           &               &           OCSVM &       0.81±0.01 &   0.81±0.0 &   0.81±0.0 &   0.81±0.0 &          X \\
           &               &            ABOD &         0.8±0.0 &   0.81±0.0 &   0.81±0.0 &   0.81±0.0 &          X \\
           &               &             SOD &        0.74±0.0 &  0.71±0.01 &   0.69±0.0 &   0.67±0.0 &          X \\
           &               &            LODA &        0.8±0.01 &   0.78±0.0 &   0.82±0.0 &   0.81±0.0 &          X \\
           &               &             COF &        0.7±0.01 &   0.68±0.0 &  0.67±0.01 &   0.65±0.0 &          X \\
           &               &  Feature-bagging &        0.92±0.0 &   0.92±0.0 &   0.91±0.0 &   0.92±0.0 &          X \\
           &               &             MCD &        0.83±0.0 &   0.84±0.0 &   0.83±0.0 &   0.83±0.0 &          X \\
           &               &            LSCP &        0.91±0.0 &   0.91±0.0 &   0.91±0.0 &   0.91±0.0 &          X \\\cmidrule{2-8}
       Red &              Green &             LOF &       0.91±0.01 &  0.92±0.01 &   0.91±0.0 &  0.91±0.01 &   0.91±0.0 \\
           &                &             ISO &        0.8±0.02 &  0.81±0.01 &    0.8±0.0 &   0.8±0.01 &    0.8±0.0 \\
           &                &           OCSVM &       0.84±0.01 &  0.85±0.01 &  0.84±0.01 &   0.84±0.0 &   0.84±0.0 \\
           &                &            ABOD &       0.73±0.02 &  0.73±0.02 &   0.72±0.0 &  0.72±0.01 &   0.72±0.0 \\
           &                &             SOD &       0.66±0.02 &  0.62±0.03 &    0.6±0.0 &  0.59±0.01 &  0.57±0.01 \\
           &                &            LODA &       0.74±0.02 &   0.8±0.01 &   0.76±0.0 &  0.79±0.01 &    0.8±0.0 \\
           &                &             COF &        0.77±0.0 &   0.7±0.01 &  0.67±0.01 &   0.63±0.0 &  0.62±0.01 \\
           &                &  Feature-bagging &       0.88±0.01 &   0.89±0.0 &   0.89±0.0 &   0.88±0.0 &   0.89±0.0 \\
           &                &             MCD &        0.8±0.02 &   0.8±0.02 &   0.78±0.0 &  0.79±0.01 &   0.79±0.0 \\
           &                &            LSCP &       0.92±0.01 &  0.93±0.01 &   0.92±0.0 &  0.92±0.01 &   0.92±0.0 \\\cmidrule{2-8}
           &             Yellow &             LOF &        0.82±0.0 &   0.81±0.0 &   0.8±0.01 &   0.81±0.0 &   0.81±0.0 \\
           &               &             ISO &        0.73±0.0 &  0.73±0.01 &  0.73±0.01 &  0.73±0.01 &   0.74±0.0 \\
           &               &           OCSVM &       0.76±0.01 &  0.77±0.01 &  0.77±0.01 &   0.77±0.0 &   0.77±0.0 \\
           &               &            ABOD &        0.74±0.0 &  0.74±0.02 &  0.74±0.01 &  0.74±0.01 &   0.74±0.0 \\
           &               &             SOD &       0.68±0.01 &  0.65±0.01 &   0.63±0.0 &   0.61±0.0 &    0.6±0.0 \\
           &               &            LODA &       0.71±0.01 &  0.72±0.01 &  0.75±0.01 &  0.73±0.01 &   0.74±0.0 \\
           &               &             COF &       0.66±0.01 &  0.63±0.01 &   0.62±0.0 &   0.61±0.0 &    0.6±0.0 \\
           &               &  Feature-bagging &       0.84±0.01 &  0.84±0.01 &  0.84±0.01 &   0.84±0.0 &   0.84±0.0 \\
           &               &             MCD &        0.78±0.0 &  0.79±0.01 &  0.78±0.01 &  0.78±0.01 &   0.78±0.0 \\
           &               &            LSCP &        0.78±0.0 &   0.77±0.0 &  0.76±0.01 &  0.77±0.01 &   0.77±0.0 \\\cmidrule{2-8}
    Yellow &              Green &             LOF &       0.83±0.01 &  0.84±0.01 &  0.84±0.01 &  0.84±0.01 &   0.84±0.0 \\
           &                &             ISO &        0.7±0.02 &  0.71±0.01 &   0.7±0.02 &  0.73±0.01 &  0.72±0.01 \\
           &                &           OCSVM &       0.75±0.02 &  0.73±0.02 &  0.74±0.01 &   0.73±0.0 &  0.73±0.01 \\
           &                &            ABOD &       0.66±0.03 &  0.68±0.02 &  0.66±0.03 &  0.69±0.01 &  0.67±0.01 \\
           &                &             SOD &       0.67±0.03 &  0.64±0.02 &   0.6±0.01 &   0.6±0.01 &  0.58±0.01 \\
           &                &            LODA &       0.67±0.02 &  0.77±0.02 &  0.72±0.02 &  0.74±0.01 &  0.75±0.01 \\
           &                &             COF &       0.74±0.02 &  0.68±0.02 &  0.68±0.01 &   0.64±0.0 &  0.62±0.01 \\
           &                &  Feature-bagging &       0.85±0.01 &   0.85±0.0 &  0.86±0.01 &   0.87±0.0 &  0.85±0.01 \\
           &                &             MCD &       0.74±0.01 &  0.75±0.02 &  0.74±0.02 &   0.76±0.0 &  0.75±0.01 \\
           &                &            LSCP &       0.78±0.01 &  0.79±0.03 &  0.78±0.02 &  0.78±0.01 &  0.78±0.01 \\\cmidrule{2-8}
           &                Red &             LOF &       0.84±0.01 &  0.83±0.02 &  0.82±0.01 &  0.81±0.01 &  0.81±0.02 \\
           &                  &             ISO &       0.62±0.03 &  0.59±0.01 &  0.58±0.01 &  0.58±0.03 &  0.58±0.03 \\
           &                  &           OCSVM &       0.72±0.02 &  0.71±0.01 &   0.7±0.01 &  0.69±0.01 &    0.7±0.0 \\
           &                  &            ABOD &        0.7±0.02 &  0.68±0.02 &  0.66±0.02 &  0.66±0.03 &  0.67±0.04 \\
           &                  &             SOD &       0.72±0.03 &  0.68±0.01 &  0.67±0.02 &  0.65±0.02 &  0.63±0.03 \\
           &                  &            LODA &        0.7±0.02 &  0.64±0.01 &  0.67±0.02 &  0.67±0.02 &  0.62±0.03 \\
           &                  &             COF &       0.82±0.02 &  0.79±0.04 &  0.75±0.01 &   0.7±0.02 &  0.68±0.02 \\
           &                  &  Feature-bagging &        0.84±0.0 &  0.83±0.01 &   0.8±0.02 &   0.8±0.01 &  0.81±0.02 \\
           &                  &             MCD &       0.77±0.02 &  0.76±0.02 &  0.74±0.02 &  0.73±0.02 &  0.74±0.03 \\
           &                  &            LSCP &       0.82±0.02 &   0.8±0.02 &   0.8±0.01 &  0.79±0.01 &  0.79±0.02 \\
      \bottomrule
\end{tabular}
}
\caption{DTLD outlier detection algorithms benchmark}
\end{table*}



\section{Experimental evaluations}\label{sec:experimental_eval} 
For our experimental evaluations we use two well-known TL datasets, i.e., BSTLD and DTLD, and MAE as a loss function as it has fixed upper and lower-bounds $[0,1]$. 
Our evaluation targets to, (a) compare various novelty scoring algorithms that fits our application, (b) evaluate usefulness of the proposed generalization score $\mathcal{G}$ and (c) interpret the notion of novelty for the datasets. 
We extracted the TL crops from both dataset to train the VAE for 750 epochs, batch size of 64, learning rate of 0.0001, $d$=32 and $\beta=0.1$. 
%\begin{table}[h]
%\centering
%\resizebox{0.3\textwidth}{!}{%
%\begin{tabular}{@{}cc@{}}
%\toprule
%Number of Epochs & 750 \\ 
%Batch size & 64 \\
%Learning rate & 0.0001 \\
%Number of Latent dimensions & 32 \\
%$\beta$ & 0.1 \\ \bottomrule
%\end{tabular}%
%}
%\caption{VAE parameters for BSTLD and DTLD datasets}
%\label{table:vaeparams}
%\end{table}

\begin{table}[h]
\centering
\resizebox{0.47\textwidth}{!}
{
\begin{tabular}{@{}ccccccc@{}}
\toprule
      & \multicolumn{2}{c}{Red} & \multicolumn{2}{c}{Yellow} & \multicolumn{2}{c}{Green} \\ \midrule
      & Train      & Test       & Train        & Test        & Train       & Test        \\
BSTLD \cite{bstld} & 3977       & 5252       & 419          & 154         & 5225        & 7454       \\
DTLD \cite{dtld}  & 19776      & 15765      & 1444         & 2946        & 25006       & 29874       \\ \bottomrule
\end{tabular}
}
\caption{TL dataset summary}
\label{table:datasets}
\end{table}
%\begin{figure}
%	\centering
%	\subfloat{\includegraphics[width=0.4 \textwidth, keepaspectratio]{bstld_umap.pdf}\label{fig:bstld_umap}} \\
%	\subfloat{\includegraphics[width=0.4 \textwidth, keepaspectratio]{driveU_umap_new.pdf}\label{fig:driveU_umap_new}}
%	\caption{2-dimensional representation of the VAE latent dimensions}
%	\label{fig:umap_tls}
%\end{figure}

\subsection{Comparative study}\label{sec:benchmark_study}
The novelty scorer is an important part of our generalisation framework (c.f. Figure \ref{fig:novelty_fw} in step {\Circled[inner color=white, outer color=blue, fill color=blue]{\textbf{d}} and {\Circled[inner color=white, outer color=blue, fill color=blue]{\textbf{e}}). 
In this section we perform a comparative evaluation of existing methods to identify a scorer that best fits our application. 
For this, we select seven novelty scoring algorithms from various paradigms (c.f. Section \ref{sec:related_work}). 
As we do not have the ground truth novelty scores for the study, we systematically engineer the datasets for our experiment. 
First we choose a contamination color, the selected color is then then removed from the train and test dataset. 
We randomly sample 10\% of contamination color samples and add them only to the test dataset. 
The added samples are novel w.r.t. training data in this context because all contamination color samples were removed from the training dataset. 
We aim to compare the ability of different novelty scoring algorithms to identify these samples in the test dataset. 
We use the implementation from PyOD and scikit-learn in our evaluation \cite{zhao2019pyod} and the area under ROC curve as a quality metric for our evaluation. 
As a randomness component is involved in our experiment, we perform the sampling three times and show the standard deviation and average ROC.

In Figure \ref{fig:benchmark}, we show the results on BSTLD and DTLD dataset with green and red as contamination colors respectively. 
Amidst the chosen scorers, LOF was the best performing (largest ROC score), followed by the KDE. 
%In order to check the stability of these two algorithms, in Figure \ref{kd_vs_lof} we increased the percentage of novel samples (2\%, 5\%, 10\%) 
However, with increase in the number of contamination (novel) samples, we observed that number false positives (normal samples identified as novel) increased more for LOF in comparison to KDE (c.f. Figure \ref{fig:lofkdbstld}). 
For this reason, we prefer to use KDE for our further experiments. 
\begin{figure}
	\centering
	\subfloat[Comparison of ROC and std. dev. of various scorers]{\includegraphics[width=0.48\textwidth, keepaspectratio]{benchmark/benchmark.pdf}\label{fig:benchmark_red_green}} \\
	\subfloat[LOF vs. KDE false positive behaviour with increasing number of novel samples]{\includegraphics[width=0.48 \textwidth, keepaspectratio]{benchmark/kd_vs_lof.pdf}\label{fig:lofkdbstld}}
	\caption{Comparative study}
	\label{fig:benchmark}
\end{figure}


\subsection{Generalization comparison for TL detector}\label{sec:generalisation_tl_comparison}
%In this section we aim to compare different CNN models using our framework in order to understand its generalization ability. 
In this section we aim to show the influence of our novelty scores on the generalization ability of the CNNs. 
However, we do not have a ground truth generalization metric for benchmarking. 
For this reason, we use various factors such as such as training iterations, batch size, learning rate and dropout rate to control the network's generalization ability. 
%We vary factors such as training iterations, batch size, learning rate and dropout rate to train multiple CNNs and study their performance on novel samples. 
As the object-under-test we chose three CNN architectures, SSD and FRCNN with inception backbone and SSD with mobilnet backbone. 
We use the density scores from the KDE as a measure of novelty, i.e., we bin the test data samples into highly novel and low novel samples by manually defined thresholds. 

%In Figure \ref{fig:nov_vs_mae} we experimentally show the effect of various factors using a similar setup as in Section \label{sec:benchmark_study}. 
%We use the density scores from the KDE as a measure of novelty, i.e., we bin the test data samples into highly novel and low novel samples by manually defined thresholds. 
From Figure \ref{fig:ssd_mobi_bs_diff} we observe that the FRCNN network with 50k iterations has an increased loss with increasing number of highly novel objects in the scene. 
One possible explanation is that the model was over-fitting the train data in comparison to the FRCNN with 20k iterations. 
Existing literature claim that increase in batch size negatively influences the generalization capacity \cite{}. On contrary, increasing learning rate has a negative impact on the network generalization capacity. 
From Figure \ref{fig:ssd_mobi_bs_diff} we infer the same as the SSD inception network with a larger batch size (10) performs worse as the number of novel samples increase. 
From Figure \ref{fig:driveu_lrr_ssd} we observe that the SSD with larger learning rate (0.0024) have a lower loss. However, the trend of loss values with increasing novelty did not change largely for the other two models. 
Finally, in Figure \ref{fig:dropout_nov} we show the effect of regularisation on the novel samples. With increasing dropout rate we see the test loss of the SSDs were smaller. 
This confirms that regularisation positively contributes for the generalisation.  

\begin{figure}
	\centering
	\subfloat[Effect of training iterations using BSTLD dataset]{\includegraphics[width=0.4\textwidth, keepaspectratio]{addl_exp/frcnn_iterations.png}\label{fig:frcnn_iterations}} \\
	\subfloat[Effect of batch size using BSTLD dataset]{\includegraphics[width=0.4 \textwidth, keepaspectratio]{addl_exp/ssd_mobi_bs_diff.png}\label{fig:ssd_mobi_bs_diff}}\\
	\subfloat[Effect of learning rate using DTLD dataset]{\includegraphics[width=0.4 \textwidth, keepaspectratio]{addl_exp/driveu_lrr_ssd.png}\label{fig:driveu_lrr_ssd}}\\
	\subfloat[Effect of dropout regularization using SSD (inception) CNN and BSTLD dataset]{\includegraphics[width=0.4 \textwidth, keepaspectratio]{addl_exp/dropout_nov.png}\label{fig:dropout_nov}}
	\caption{Effect of various factors on the loss function}
	\label{fig:nov_vs_mae}
\end{figure}
Although we used manual thresholds in our above experiments, out generalization score does not require it. The novelty scores are used directly as weights for the loss values. 

As a generalization scoring metric, we compare our method with test data accuracy. 
Conventionally the generalization of a CNN is often evaluated based on test data accuracy. 
%To understand its behaviour better, we compare the generalisation ability of the SSD for varying learning rates on entire datasets (without categorizing into levels). 
For this, we trained SSDs at five learning rates on the two datasets separately. 
That is, in total we have 10 SSDs trained, the training parameters and the trained models are made available for reproducible results\textsuperscript{\ref{note1}}. 
We then compare the generalisation ability of these two detectors using the test data accuracy (True positive$=IoU\geq0.5$), our method of novelty weighted loss and just the average loss without novelty weighting. 
Like outliers, novel samples are also infrequent in a dataset. 
To avoid the effect of the imbalance in the number of novel and normal samples we categorize (c.f. Figure \ref{fig:split_bstld_intohml}) the novelty scores into three quantile buckets, i.e., high, medium and low, and sample 100 images from each category. 
The density score of KDE is inversely proportional to novelty \footnote{We normalise the density scores as weights to avoid negative weights.
The implementation details are available in: http://share.com.\label{note1}}. 
\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{split_bstld_intohml.pdf}
\caption{Categorize the density scores into novelty levels}
\label{fig:split_bstld_intohml}
\end{figure}
Comparing test data accuracy as a measure of generalisation, it is easy to state that FRCNN generalizes better on BSTLD dataset from Table \ref{tab:generalization}. 
However, from Figure \ref{fig:compare_detector_bstld} we see that the loss values of FRCNN detector is much smaller in comparison to the SSD. 
\begin{table}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{@{}ccccc@{}}
\toprule
Dataset & Network & Accuracy & $\mathcal{G}$ & 1-MAE (no weighting) \\ \midrule
\multirow{2}{*}{BSTLD} & SSD & 0.62 & 0.3 & 0.37 \\ %TP(hml) = (38.0, 79.0, 69.0)
 & FRCNN & 0.6 & 0.51 & 0.50 \\ \hline %TP(hml)=(53.0, 63.0, 65.0)
\multirow{2}{*}{DriveU} & SSD & 0.28 & 0.44 & 0.23 \\ %(58.0, 61.0, 52.0) 
 & FRCNN & 0.46 & 0.64 & 0.42 \\ \bottomrule %(39.0, 56.0, 51.0) 
\end{tabular}
}
\caption{Comparing test data accuracy with our generalization score and MAE without novelty weights}
\label{tab:generalization}
\end{table}
\begin{figure}
\centering
\subfloat{\includegraphics[width=0.36\textwidth, height=6cm]{ssd.png}\label{fig:ssd_bstld_compare}} \\
\subfloat{\includegraphics[width=0.36\textwidth, height=6cm]{frcnn.png}\label{fig:frcnn_bstld_compare}}
\caption{SSD vs. FRCNN on BSTLD dataset}
\label{fig:compare_detector_bstld}
\end{figure}
This is also inferred from the non-weighted average loss value in Table \ref{tab:generalization}. 
In comparison to the average loss without any weighting our novelty weighted loss $\mathcal{G}$ rewards the FRCNN for its prediction performance on the novel samples.
On contrary, SSD predictions have a higher loss on both high and medium samples. 
Hence, after penalization our $\mathcal{G}$ score is smaller in comparison to the un-weighted 1-MAE value. 

Conventionally the generalization of a CNN is evaluated based on test data accuracy. 
To understand its behaviour better, we compare the generalisation ability of the SSD for varying learning rates on entire datasets (without categorizing into levels). 
For this, we trained SSDs for TL localization at five learning rates on the two datasets separately. 
That is, in total we have 10 SSDs trained, the training parameters and the trained models are made available for reproducible results\textsuperscript{\ref{note1}}. 
%Hence, in Figure \ref{fig:generalization_benchmark_ssd_bstld_lrr_10k} we compare the generalisation of the CNNs using our method and test data accuracy. 
From Figure \ref{fig:bstld_ssd_lr} and \ref{fig:driveu_ssd_lr}, we see that our scoring methodology is comparable to the test data accuracy. 
However, on the DTLD dataset we observe that the models with learning rate 0.0006 and 0.0012 do not agree with each other. That is the test accuracy infers that the SSD with learning rate of 0.0006 is better than the other. However, our score contradicts this inference. 
In addition, using the average loss (without novelty weighting) we observed that both models had very similar values of 0.24 and 0.25 respectively. 
However, on evaluating their distribution of loss over the novelty values we observed that the SSD with a learning rate of 0.012 was performing well on high and medium samples in addition to the low novelty ones. 
It is for this reason our generalization assigns the SSD with learning rate of 0.0012 comparatively better score.

\begin{figure}
\centering
\subfloat[BSTLD]{\includegraphics[width=0.45\textwidth]{generalization_benchmark_ssd_bstld_lrr_10k.pdf}\label{fig:bstld_ssd_lr}} \\
\subfloat[DTLD]{\includegraphics[width=0.45\textwidth]{driveu_loc/driveu_gen_vs_tac.pdf}\label{fig:driveu_ssd_lr}}
\caption{Comparing test data accuracy with our generalization score}
\label{fig:generalization_benchmark_ssd_bstld_lrr_10k}
\end{figure}
\begin{figure}
\centering
\subfloat[SSD learning rate = 0.0006]{\includegraphics[width=0.4\textwidth]{driveu_loc/ssd_6_checkdriveu.pdf}\label{fig:ssd_06_checkdriveu}} \\
\subfloat[SSD learning rate = 0.0012]{\includegraphics[width=0.4\textwidth]{driveu_loc/ssd_12_checkdriveu.pdf}\label{fig:ssd_12_checkdriveu}} 
\caption{Comparing test data accuracy with our generalization score}
\label{fig:dtld_06_vs_12}
\end{figure}


\subsection{Interpretation of novelty}\label{sec:interpretation}
In the previous sections, we used the word novelty to describe objects that are not normal w.r.t. the training dataset. However, in practical applications the user needs to interpret novelty to further enrich the dataset or improve the CNN architecture. 
Therefore, in this section we aim to understand the latent dimensions because the KDE scores novelty based on them. 
Instead of visualizing all the latent dimensions, we used mutual information \cite{reza1994introduction} to select those dimensions that best classifies the samples into high and low novelty categories (c.f. Figure \ref{fig:split_bstld_intohml}). 
By this way we selected the dimensions that regulate the novelty of the datasets. 
In Figure \ref{fig:bstld_rel_traversals_bstld} and \ref{fig:driveu_red_green_yel_redyel_pc} we visualize the traversal (low to high values) of the top dimensions on BSTLD and DTLD datasets respectively. 
We understand that the dimensions represent various human-interpretable properties of the image, viz., brightness, color shade, inlay or the bulb size. 
\begin{figure}
	\centering
	\subfloat[$z_{9}$ controls the size of the traffic light bulb]{\includegraphics[width=0.47\textwidth]{bstld_green_traversal_d9.jpg}\label{fig:bstld_green_traversal_d9}} \\
	\subfloat[$z_2$ controls the background brightness]{\includegraphics[width=0.47\textwidth]{bstld_red_traversal_d2.jpg}\label{fig:bstld_red_traversal_d2}} \\
	\subfloat[$z_{19}$ controls the traffic light inlay]{\includegraphics[width=0.47\textwidth]{bstld_red_arrow_19.png}\label{fig:bstld_red_arrow_19}} \\
	\caption{Traversal of latent dimension for a VAE trained on BSTLD dataset}
	\label{fig:bstld_rel_traversals_bstld}
\end{figure}
\begin{figure}
	\centering
	\subfloat[$z_{10}$ controls the white spot on the green traffic light]{\includegraphics[width=0.47\textwidth]{driveu_loc/driveu_green10_traversal_whitespot.png}\label{fig:driveu_green10_traversal_whitespot}} \\
	\subfloat[$z_{20}$ controls the shade of red color light]{\includegraphics[width=0.47\textwidth]{driveu_loc/driveu_red_20.png}\label{fig:driveu_red_20}} \\
	\subfloat[$z_{23}$ controls the blurriness of the red yellow light]{\includegraphics[width=0.47\textwidth]{driveu_loc/driveu_red_yelow_23.png}\label{fig:driveu_red_yelow_23}}\\
	\subfloat[$z_{5}$ controls the shades of yellow color light]{\includegraphics[width=0.47\textwidth]{driveu_loc/driveu_yellow5_traversal.png}\label{fig:driveu_yellow5_traversal}}
	\caption{Traversal of latent dimension for a VAE trained on DriveU dataset}
	\label{fig:rel_traversals_driveu}
\end{figure}
\begin{figure*}
	\centering
	\subfloat{\includegraphics[width=0.47 \textwidth, keepaspectratio]{bstld_green_pc_kde.png}\label{fig:bstld_green_pc_kde}}
	\subfloat{\includegraphics[width=0.47 \textwidth, keepaspectratio]{bstld_red_pc_kde.png}\label{fig:bstld_red_pc_kde}}
	\caption{Visualization of sample novelty based on KDE density scores for green (left) and red (right) traffic lights in BSTLD dataset}
	\label{fig:bstld_red_green_pc}
\end{figure*}
%Driveu
\begin{figure*}
	\centering
	\subfloat{\includegraphics[width=0.47 \textwidth, keepaspectratio]{driveu_loc/driveu_green_all.png}\label{fig:driveu_green_all}}
	\subfloat{\includegraphics[width=0.47 \textwidth, keepaspectratio]{driveu_loc/driveu_red_yell_all.png}\label{fig:driveu_red_yell_all}}\\
	\subfloat{\includegraphics[width=0.47 \textwidth, keepaspectratio]{driveu_loc/driveu_red_all.png}\label{fig:driveu_red_all}}
	\subfloat{\includegraphics[width=0.47 \textwidth, keepaspectratio]{driveu_loc/driveu_yellow_all.png}\label{fig:driveu_yellow_all}}
	\caption{Visualization of sample novelty based on KDE density scores for green (top-left), red (top-right), red-yellow (bottom-left) and yellow (bottom-right) traffic lights in DriveU dataset}
	\label{fig:driveu_red_green_yel_redyel_pc}
\end{figure*}
In Figure \ref{fig:bstld_red_green_pc} and \ref{fig:rel_traversals_driveu} we map the data samples on the traversal using parallel coordinates. 
Although we trained the detector for localization and not classification, we evaluate class-wise novelty as we found them to be more straightforward. However, the scoring was done over all colors at one shot and not class-wise. 
In Figure \ref{fig:bstld_red_green_pc} we show the green and red TL samples of BSTLD dataset. 
We infer that dimension $z_9$ influences the novelty of green lights, i.e., smaller values of $z_9$ are scored as high novel samples. 
From our traversal study on $z_9$ in Figure \label{fig:bstld_green_traversal_d9} we interpret that it controls the size of the light bulb. 
That is, the $z_9$ is inversely proportional to the bulb size or the training data has more of smaller traffic lights. 
This leads to the KDE assigning larger lights as more novel objects. 
The $z_2$ dimension is commonly influencing the novelty in green and red lights, from Figure \ref{fig:bstld_red_traversal_d2} we understand that it controls the background brightness. 
The novelty scorer assigns the TLs with bright background as more novel. 
Similarly, for red TLs in Figure \ref{fig:bstld_red_green_pc}, we observe that the smaller value of $z_19$ is more novel. 
The dimension $z_19$ controls the inlay, as we increase the value from left to right the image changes from a left facing arrow to red circled inlay (c.f. Figure \ref{fig:bstld_red_arrow_19}). 
From the perspective of human-interpretation, this means that the training dataset had fewer arrow inlays compared to the circle inlays. 

Likewise, we performed the study of interpretation in the DTLD dataset for four different TL colors. 
From Figure \ref{fig:driveu_red_green_yel_redyel_pc} we observe that novelty increases with increase in $z_{10}$ or $z_5$. 
From Figure \ref{fig:rel_traversals_driveu}, we understand that $z{10}$ controls the traffic light size, but also a bright spot around it. 
These large TLs with such glaring white spots are deemed novel by the KDE. 
The $z_5$ dimension seem to control the shade of red, as we traversed to higher values we observed that the color was much darker. 
On contrary, the novelty of samples increase with the decrease of $z_{20}$ and $z_{23}$. 
The $z_{20}$ dimension regulates the blurriness of the lights, whereas, the $z_5$ was responsible for the shade of yellow light. 
With increase in $z_5$ we observed that the yellow shade was much stronger that it tends to look more red in color and also the size of the light grew in size. 




\begin{algorithm}[h]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{Computing $\mathcal{G}$ score of CNN $m$ on $\mathcal{D}_{te}$}
\begin{algorithmic}[1] 
		\Require $\mathcal{D}_{tr}$, $Y_{tr}$, $\mathcal{D}_{te}$,$Y_{te}$, $e_\phi$ 
		\If{\text{training phase}} 
		\State $\textbf{Z}= zeros(N_{tr}, m)$ \label{line:start_train}
		\For{$i \in [1:N_{tr}]$}
		\State $\textbf{Z}_{i*} = e_\phi(I_i \in \mathcal{D}_{tr})$
		\EndFor
		\State $outlier\_detector = fit\_kde(\textbf{Z})$ \label{line:end_train}
		\EndIf
		\If{\text{testing phase}}
		\State $\textbf{Z}= zeros(N_{te}, m)$ \label{line:start_test}
		\For{$i \in [1:N_{te}]$}
		\State $\textbf{Z}_{i*} = e_\phi(I_i \in \mathcal{D}_{te})$
		\EndFor
		\State $scores = score\_novelty(\textbf{Z})$\label{line:end_test}
		\State $\hat{Y} = m(\mathcal{D}_{te})$
		%\State $loss = \mathcal{L}(Y,\hat{Y})$
		\State $\mathcal{G}= \frac{\sum_{i=1}^{N}scores_i \cdot  (1-\mathcal{L}(Y_i,\hat{Y}_i))}{\sum_{i=1}^{N}scores_i}$\label{line:score_samples}
		\EndIf
\end{algorithmic}
	\Return $\mathcal{G}$
	\label{alg:generation}
\end{algorithm}



\author{\IEEEauthorblockN{Anonymous1}
\IEEEauthorblockA{\textit{Anonymous1} \\
Anonymous1 \\
Anonymous1}
\and
\IEEEauthorblockN{Anonymous2}
\IEEEauthorblockA{\textit{Anonymous2} \\
Anonymous2 \\
Anonymous2}
\and
\IEEEauthorblockN{Anonymous3}
\IEEEauthorblockA{\textit{Anonymous3} \\
Anonymous3 \\
Anonymous3}
}





==> problem_overview.tex <==
\section{Problem and Notation Overview}
In this section we formally define the addressed problem. 
Assume an image dataset $\mathcal{D}$ with $N$ images, where $I\in\mathcal{D}$. 
The target object, e.g., traffic light, is annotated by a bounding-box\footnote{\label{numDet}For the sake of simplicity we assume each image $I$ has only one bounding box. However, there can be multiple bounding boxes per image.} which is a list of four coordinates. 
The collection of annotations for all images in $\mathcal{D}$ is denoted as $Y=(y_1,\cdots,y_N)$. 
%Each bounding-box $y_i \in Y$ is linked to a class $c\in \mathcal{P}$ from a set of all classes associated with the dataset. 
%The collection of all classes associated to the annotations is denoted as $C=(c_1,\cdots,c_N)$
A pre-trained CNN detector $m: \mathcal{D}\mapsto (\hat{Y}, S)$ fed with the dataset returns $N$ predicted bounding boxes and its corresponding confidence scores $S=s_1,\cdots,s_N$, where, $s \in \mathbb{R}$. With the ground truth and the predicted detections available, the goodness of a CNN can be estimated using a simple loss function, $\mathcal{L}:(Y,\hat{Y},S)\mapsto \mathbb{R}$.
The test dataset will follow the same structure as the training data. To avoid redundant definitions the test and train data will be denoted with the subscript $te$ instead of $tr$ respectively. That is, $\mathcal{D}_{te}$ and $\mathcal{D}_{tr}$ denotes the test and train datasets respectively. 

For the given testing dataset and its annotations, we aim to score the novelty of each object $y\in Y_{te}$ w.r.t. the objects $Y_{tr}$ in the training dataset $\alpha:(y_{te},Y_{tr})\mapsto N \in \mathbb{R}.$
The generalization score of the CNN is estimated based on the goodness the detector $m$ on highly novel test objects. That is, the generalization score will target the network's performance on novel samples to evaluate its ability to handle deviations from the training data $\mathcal{G}:(N, \mathcal{L})\mapsto \mathbb{R}.$

